Uncertainty-Aware Velocity Correction for Proprioceptive Vehicle Localization using Evidential Mamba

Reliable localization in GNSS-denied environments remains a fundamental challenge for intelligent vehicles, as inertial navigation systems accumulate unbounded drift without external correction. Existing approaches provide drift correction through dedicated infrastructure, expensive external sensors, or complex multi-sensor fusion, each introducing practical deployment barriers. We propose Evidential Velocity Correction using Mamba (EVC-Mamba), a learning-based architecture that transforms onboard vehicle sensor data into a virtual velocity sensor for IMU drift correction without additional hardware. A Mamba-based selective state space model captures the temporal dynamics of vehicle motion, while evidential deep learning with a Normal-Inverse-Gamma distribution provides principled uncertainty quantification. The resulting uncertainty-aware velocity estimate is incorporated as a virtual correction measurement into an Error-State Extended Kalman Filter to reduce position drift. Evaluation on real-world vehicle data demonstrates that inertial navigation using the proposed velocity correction achieves localization accuracy within 10% of a dedicated external velocity sensor across different outage durations. The proposed architecture supports real-time onboard deployment at 40 Hz on edge hardware, enabling reliable localization during prolonged GNSS outages.

==> backup.tex <==
\section{Introduction}
%Comprehensive Motivation
%State-of-the-art Overview
%Clear Gap Identification
%Method Summary
%Explicit Contributions
Accurate localization is a key requirement for the safe and reliable operation of intelligent vehicles, enabling essential functions such as path planning, motion control, and \gls{adas}~\cite{intro_localization}.
In general, precise localization is achieved by fusing an inertial navigation system (\gls{imu}) with \gls{gnss} signals to compensate for drift~\cite{gnss}. 
However, in \gls{gnss}-denied indoor environments, such as parking structures and tunnels, the position drift grows unbounded due to the absence of external corrections~\cite{lstmIMU}.

The state-of-the-art methods in indoor localization can be broadly categorized into \gls{rf}-based approaches, inertial navigation systems, vision-based methods, and multi-sensor fusion techniques~\cite{indoor_survey}. 
\gls{rf}-based methods are widely utilized in indoor positioning. However, their performance relies on dedicated infrastructure and can degrade due to signal attenuation and multipath effects~\cite{rf-based}. 
Exteroceptive vision-based approaches using cameras and LiDARs can achieve good accuracy, but their performance is sensitive to illumination variations and occlusions, which may lead to feature tracking failures~\cite{localisation_survey}. 
Multi-sensor fusion techniques improve robustness by combining complementary modalities~\cite{vio_eccv,vins,lidar_imu_gnss}, yet they often increase system complexity and cost. 
While \gls{imu}-based inertial positioning systems offer a low-cost, proprioceptive solution, they are prone to drift due to sensor noise and bias accumulation~\cite{noise_imu}.
Among these methods, \gls{imu}s are particularly attractive for infrastructure-free indoor localization, motivating research into GNSS-independent correction techniques to reduce drift.

\begin{figure}[tb]
    \centering
        \includegraphics[scale=1.25, trim=10pt 10pt 10pt 10pt, clip]{images/ipin_firstpage (1).pdf}
    %\caption{Overview of the test vehicle configuration and \gls{piml2} architecture for proprioceptive localization.}
    \caption{Overview of the test vehicle configuration and the proposed \textcolor{red}{evimamba} velocity correction for \gls{imu}-based proprioceptive localization.}
    \label{fig:piml_architecture}
    \vspace{-0.5cm}
\end{figure} %note{arrows and hybrid fusion}

Recently, data-driven methods have improved \gls{imu}-based dead reckoning~\cite{lstmIMU,noise_imu}. Their effectiveness is still limited to short GNSS outages, as external correction is required to constrain long-term drift~\cite{imu_survey}. 
External velocity sensors provide a GNSS-independent correction signal for \gls{imu}s and enable improved long-term performance in indoor environments. However, such approaches require additional hardware, such as Correvit sensors~\cite{wheel-imu}. Readily available onboard vehicle sensors, e.g., steering wheel angle and wheel speed measurements, offer a promising alternative for virtual velocity estimation~\cite{abinav,sven}. Existing model-based approaches compute velocity from onboard sensor data using vehicle dynamic models~\cite{onboardsensors-velocity}, which are often insufficient for complex vehicle dynamic maneuvers.

%Finally, an \gls{ekf} incorporates the uncertainty-aware velocity correction along with \gls{imu} measurements to improve vehicle localization accuracy in GNSS-denied environments. The proposed architecture is real-time capable and achieves performance similar to that of external velocity correction sensors without additional cost. 

To address these limitations, this work introduces \gls{evimamba}, a novel learning-based architecture for precise \gls{imu} velocity correction using onboard vehicle sensors, as illustrated in Fig. 1.
%To address these limitations, this work introduces \acrshort{evimamba}, a novel \textbf{Evi}dential Velocity Correction using Selective State-Space Models (\textbf{Mamba}) for \textbf{I}nertial \textbf{N}avigation using onboard vehicle sensors, as illustrated in Fig. 1.
It employs a selective~\gls{ssm} based on Mamba~\cite{mamba} to estimate vehicle velocity, while uncertainty in the estimates is captured using evidential deep learning via a \gls{nig} distribution.
The uncertainty-aware velocity correction is then integrated as a virtual measurement within an~\gls{ekf}, together with \gls{imu} measurements, to improve vehicle localization accuracy in GNSS-denied environments.
By leveraging data-driven learning together with uncertainty modeling, our approach can capture nonlinear vehicle dynamics and provide robust velocity correction even under complex driving maneuvers. 
The proposed architecture is real-time capable and achieves performance comparable to external velocity correction sensors, without additional cost. The main contributions of this work are as follows:
\begin{itemize}
\item \gls{gnss}-Independent velocity correction for \gls{imu}-based indoor localization using onboard sensors.
\item Uncertainty-Aware robust velocity estimation using Mamba-\gls{ssm} and evidential deep learning. 
\item Horizontal-frame IMU mechanization with uncertainty-aware velocity correction in an \gls{ekf}.
\item Real-time capability with performance comparable to Correvit class sensors. 
\end{itemize}

\section{Related works V1}
Existing proprioceptive localization approaches can be broadly categorized into classical Bayesian filter-based methods and data-driven \gls{ml} methods.

Recursive Bayesian filter-based approaches for dead-reckoning, such as the \gls{kf}, \gls{ekf}, Error-State \gls{ekf}, and particle filters, leverage motion models for vehicle state estimation and fuse these with \gls{imu} measurements for localization~\cite{survey_localization}. Although these methods generalize well, they are vulnerable to complex, multifaceted noise that degrades localization accuracy over time~\cite{lstmIMU,noise-imu-degrade}. Adaptive filters~\cite{adaptive_kalman} strive to address this by varying the process or measurement noise covariance matrices. Nevertheless, \gls{imu}-based dead reckoning remains prone to quadratic growth of position error over time, caused by the accumulation of measurement noise through double integration of acceleration data~\cite{lstmIMU}. To reduce this drift, additional sensors can provide velocity information. For example, in~\cite{wheel-imu}, the authors improved 2D \gls{imu}-based dead reckoning by utilizing velocity measurements from a wheel-mounted \gls{imu}, which reduced pose drift from quadratic to linear rate. Similarly, onboard sensors such as wheel speed and steering wheel angle can be used to estimate vehicle velocities through vehicle dynamic models~\cite{onboardsensors-velocity}. However, complete onboard sensor-based localization is fundamentally constrained by the assumptions of the vehicle motion models, which hold only under certain driving conditions~\cite{icra_wheelodometry}. 

Data-driven proprioceptive localization approaches employ \gls{ml} techniques to calibrate \gls{imu} measurements~\cite{imu_calibrate}, correct integration drift~\cite{deep_position}, and adaptively compensate for sensor noise~\cite{adaptive_noise_israel,noise_imu}.  
In~\cite{calibnet2022}, deep learning was used to enhance the performance of low-cost \glspl{imu} and mimic the output characteristics of high-grade sensors. 
Although \gls{ml}-based methods have been widely explored for handling stochastic noise in \gls{imu}-based localization, their application to onboard odometry has been less studied. Recent works~\cite{abinav,TUdelft} demonstrate the potential of combining onboard sensors with \gls{ml} techniques, showing that \gls{ml} models can transform onboard measurements into accurate vehicle dynamic state estimates without complex vehicle dynamics models.

Evidential deep learning has recently emerged as a principled framework for modeling predictive uncertainty in neural networks without relying on costly sampling or ensemble techniques. Instead of producing point estimates, evidential approaches parameterize higher-order probability distributions, such as the normal-inverse-gamma (NIG), to jointly estimate mean and uncertainty~\cite{sensoy2018evidential,evidential_regression}. This allows models to distinguish between aleatoric and epistemic uncertainty in a single forward pass. Such properties are particularly valuable in safety-critical applications like autonomous driving, where unreliable predictions must be identified and handled appropriately. Recent works have applied evidential learning to perception and mapping tasks, including uncertainty-aware sensor fusion and evidential occupancy grid mapping for autonomous systems~\cite{capellier2021fusion,geletu2024evidential}.  
These approaches demonstrate improved robustness under noisy and out-of-distribution conditions, and enable more consistent integration with probabilistic frameworks. Despite these advantages, the use of evidential deep learning for modeling uncertainty in learned proprioceptive velocity estimation and its integration into recursive state estimation pipelines remains largely unexplored.

Recently, sequence modeling architectures based on structured state space models (SSMs) have gained attention as efficient alternatives to recurrent and attention-based networks. In particular, the Mamba architecture~\cite{mamba} introduces a selective state space mechanism that enables linear-time sequence modeling while retaining strong long-range dependency modeling capabilities. Compared to transformers, Mamba avoids quadratic complexity and exhibits improved scalability for long temporal sequences, making it well-suited for high-frequency sensor data such as \gls{imu} and vehicle signals. Prior works have demonstrated the effectiveness of SSM-based models, including S4~\cite{gu2021efficiently} and its variants, in time-series forecasting and control applications. More recently, Mamba has been applied to diverse domains such as audio processing, vision, and robotics, showing competitive or superior performance to transformer-based approaches~\cite{mamba}. Despite these advances, the use of Mamba architectures for vehicle state estimation and sensor fusion in localization remains an emerging area, with limited exploration in the context of onboard proprioceptive sensing.

Modeling temporal dependencies in vehicle state estimation has traditionally relied on recurrent neural networks, with approaches such as IONet~\cite{ionet} and RoNIN~\cite{ronin} demonstrating the potential of LSTM-based architectures for inertial odometry. More recently, transformer-based models have been adopted for autonomous driving tasks, leveraging attention mechanisms for multi-sensor fusion and long-range temporal reasoning~\cite{transfuser,bevformer}. However, both recurrent and attention-based architectures suffer from limitations in capturing long sequences efficiently, particularly for high-frequency signals such as \gls{imu} and onboard vehicle data. Structured state space models (SSMs), including S4~\cite{gu2021efficiently} and its variants, have been proposed as an alternative, offering linear-time complexity while retaining strong sequence modeling capabilities. Building on this line of work, the Mamba architecture~\cite{mamba} introduces a selective state space mechanism that enables content-dependent sequence modeling with improved efficiency and scalability. While these models have shown promising results in domains such as language, vision, and audio processing, their application to vehicle dynamics modeling and proprioceptive localization remains limited. In particular, the combination of SSM-based architectures with uncertainty-aware learning for robust velocity estimation has not yet been fully explored.

In this work, we address these limitations by combining the strengths of classical filtering and data-driven learning through the proposed \gls{piml2} architecture for onboard proprioceptive odometry. While orthogonal to multi-sensor fusion, the proposed framework can be integrated with such approaches by incorporating additional sensing modalities.  


\section{Related works V2}
Proprioceptive localization for ground vehicles is commonly addressed using recursive Bayesian filtering methods such as the \gls{kf}, \gls{ekf}, Error-State \gls{ekf}, and particle filters~\cite{survey_localization}. 
These approaches fuse motion models with \gls{imu} measurements to estimate vehicle states, but suffer from drift due to noise accumulation, leading to quadratic growth of position error over time~\cite{lstmIMU,noise-imu-degrade}.
To mitigate this, additional precise velocity measurements from external sensors or wheel-mounted \gls{imu}s have been incorporated, reducing drift to linear growth~\cite{wheel-imu}.
Alternatively, vehicle velocities can be inferred from onboard signals such as wheel speeds and steering angles using kinematic models~\cite{onboardsensors-velocity}. 
However, such approaches rely on simplifying assumptions that are often violated in real-world driving conditions, limiting their robustness~\cite{icra_wheelodometry}. 
% Adaptive filtering methods partially address modeling errors but do not eliminate these fundamental limitations~\cite{adaptive_kalman}.

Learning-based methods have recently been explored to improve inertial navigation by calibrating IMUs, compensating drift, and modeling sensor noise~\cite{imu_calibrate,deep_position,adaptive_noise_israel,noise_imu}. 
In~\cite{calibnet2022}, deep learning was used to enhance the performance of low-cost \glspl{imu} and mimic the output characteristics of high-grade sensors. 
While most prior work focuses on IMU signals, recent studies~\cite{abinav,TUdelft} demonstrate that machine learning models can map onboard vehicle measurements directly to dynamic states, bypassing explicit vehicle models.

In parallel, uncertainty-aware learning has gained attention for safety-critical systems. 
Evidential deep learning enables joint estimation of predictive mean and uncertainty by parameterizing higher-order distributions such as the Normal-Inverse-Gamma~\cite{sensoy2018evidential,evidential_regression}, and has shown improved robustness in perception and mapping tasks~\cite{capellier2021fusion,geletu2024evidential}. However, its application to proprioceptive precise velocity estimation and integration into recursive state estimation remains underexplored.

Modeling temporal dependencies in sequential sensor data has traditionally relied on recurrent architectures such as LSTMs, as used in inertial odometry frameworks like IONet and RoNIN~\cite{ionet,ronin}.
Transformer-based models have further improved long-range temporal reasoning and multi-sensor fusion~\cite{transfuser,bevformer}, but incur high computational cost for long sequences. 
Structured State Space Models (SSMs), including S4~\cite{gu2021efficiently}, offer an efficient alternative with linear-time complexity.
The recently proposed Mamba architecture~\cite{mamba} extends this line of work with selective state space modeling, enabling scalable and expressive sequence learning. 
Despite their advantages, SSM-based models have seen limited adoption in vehicle state estimation and proprioceptive localization.

Existing approaches thus fail to jointly address learning-based precise velocity estimation from onboard signals, principled uncertainty quantification, and efficient sequence modeling within a unified probabilistic framework. 
In this work, EviMamba-INS is proposed, which combines a Mamba-based precise virtual velocity sensor with evidential deep learning for uncertainty estimation and integrates the resulting predictions into an Error-State~\gls{ekf}.
This enables robust, drift-bounded localization in \gls{gnss}-denied environments without reliance on external sensors.



